On Shapley Credit Allocation for Interpretability

We emphasize the importance of asking the right question when interpreting the decisions of a learning model. We discuss a natural extension of the theoretical machinery from Janzing et. al. 2020, which answers the question "Why did my model predict a person has cancer?" for answering a more involved question, "What caused my model to predict a person has cancer?" While the former quantifies the direct effects of variables on the model, the latter also accounts for indirect effects, thereby providing meaningful insights wherever human beings can reason in terms of cause and effect. We propose three broad categories for interpretations: observational, model-specific and causal each of which are significant in their own right. Furthermore, this paper quantifies feature relevance by weaving different natures of interpretations together with different measures as characteristic functions for Shapley symmetrization. Besides the widely used expected value of the model, we also discuss measures of statistical uncertainty and dispersion as informative candidates, and their merits in generating explanations for each data point, some of which are used in this context for the first time. These measures are not only useful for studying the influence of variables on the model output, but also on the predictive performance of the model, and for that we propose relevant characteristic functions that are also used for the first time.

==> contributions.tex <==
\textbf{Contributions.} Our first focus has been on establishing the technical differences in the characteristic functions for the computation of Shapley values, which result in significantly diverse implications in terms of the nature of interpretations which are of three types, \textit{observational}, \textit{model specific}, and \textit{causal}. It is important to note that different use cases call for the application of the previously mentioned different variants. 

We also show how these differences are applicable when we use various measures of interpretation in the design of characteristic functions for computing Shapley values. Besides the commonly used expected value of the scoring function of the model, we also discuss measures of statistical uncertainty and dispersion as informative candidates, and their merits, some of which have been used in this context for the first time, in generating explanations for each datapoint. 

These measures are not only useful for studying the influence of variables on the model output, but also on the predictive performance of the model, and to that end, we propose relevant characteristic functions which are also used for the first time. 
%
%Our second focus has been in studying different value functions. The most commonly known SHAP \cite{lundberg_shap,shap}, generates additive feature attributions towards explaining the model scoring function. On a related note, it would also be useful to understand the involvement of the features towards an improvement or degradation in the model performance. \cite{sage} does this by identifying features influential towards the model loss at a global level. We assert that the local interpretation of the same is in fact a trivial application of the Shapley concept to the per sample loss. 
%
%Therefore it turns out that in most cases the problem of interpretability entails the understanding of the influence of a variable towards a real valued output which could be the softmax output of a classifier, or the prediction by a regressor or even real valued loss functions such as cross entropy and mean squared errors. Influence can be measured from different statistical perspectives. The most well known one is the influence of a variable towards the deviation of the real valued output from the average. Another variant is from an information theoretic perspective, in which the influence of a variable towards reducing the entropy of a real valued output is measured \cite{c-shapley,janzing-cic}. 
%
%Shannon entropy ($H$) measures the uncertainty in a random variable where the notion of uncertainty captures the lack of predictability of a variable. A discrete random variable for which the symbols do not possess an ordering naturally begets this definition and the entropy is maximized by a uniform distribution over the symbols. However consider the continuous valued case where the symbols are ordered and for the sake of argument let us assume the symbols restricted to $[0,1]$. In this case, a scenario of no information i.e. the uniform distribution is of less uncertainty than an extremely polarized distribution which leaves us even more confused. For example, let the random variable denote a score between 0 and 1 as the probability of rain today. In such a scenario having weights of 0.5 on both the extreme ends i.e, 0 and 1, is the most confusing scenario. 
%
%Statistical measures of dispersion such as the cumulative paired Shannon entropy ($\mathcal{E}$) \cite{klein-1,klein-2} capture this notion of contradictory information in the form of assigning higher entropies to a more polarized distribution. $\mathcal{E}$ in particular has been unknowingly applied in several unrelated contexts such as in fuzzy set theory, uncertainty theory, dispersion theory for discrete ordered data as well as in reliability theory. \cite{klein-1,klein-2} formalize this measure by drawing parallels to its information theoretic counterparts, namely divergence, entropy and mutual information. \cite{klein-1} derives the maximum entropy distributions under different constraints for $\mathcal{E}$ and formulates rank tests using the measure which coincidentally reduces to well known rank tests from the literature as a specialization. 


==> headers_copy.tex <==
\usepackage[T1]{fontenc}
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{calc}
\usetikzlibrary{snakes}
\usepackage{cite}
\usepackage{graphicx}
\usepackage{array}
\usepackage{mdwmath}
\usepackage{mdwtab}
\usepackage{eqparbox}
\usepackage{fixltx2e}
\usepackage{url}
\usepackage{pgf}
\usepackage{lipsum}
\usepackage{multirow}
\usepackage{subcaption}
%\usepackage[cmex10]{amsmath}
\usepackage{amsfonts,amssymb,amsthm}
\usepackage{xspace}
\usepackage{xcolor}
%\usepackage{algorithmic}
\usepackage{bm}
\usepackage{bbm}
\usepackage{booktabs}
\usepackage{etoolbox}
\usepackage{makecell}
\usepackage{nicefrac}
\usepackage{textcomp}
\usepackage{stmaryrd}
\usepackage{mathrsfs}
\usepackage{paralist}
\usepackage{comment}

\usepackage[font=footnotesize,labelsep=space,labelfont=bf]{caption}

%\usepackage[colorlinks=true,urlcolor=blue]{hyperref}
\usepackage{url}

\hyphenation{op-tical net-works semi-conduc-tor}

\usepackage[pdftex,bookmarks=true,pdfstartview=FitH,colorlinks,linkcolor=blue,filecolor=blue,citecolor=blue,urlcolor=blue,pagebackref=false]{hyperref}
    \urlstyle{sf}

%\usepackage[draft]{hyperref}
%\usepackage{url}


\makeatletter
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother



\newtheorem{theorem}{Theorem}%[chapter]
\newtheorem*{theorem*}{Theorem}
\newtheorem{definition}{Definition}%[chapter]
\newtheorem{lemma}{Lemma}%[chapter]
\newtheorem*{lemma*}{Lemma}
\newtheorem{claim}{Claim}%[chapter]
\newtheorem{corollary}{Corollary}%[chapter]
\newtheorem*{cor*}{Corollary}
\newtheorem{remark}{Remark}%[chapter]
\newtheorem{fact}{Fact}%[chapter]

\newcommand{\TODO}[1]{{{\color{red}#1}}}
\newcommand{\CHECK}[1]{{{\color{blue}#1}}}
\newcommand{\CHECKM}[1]{{{\color{magenta}#1}}}

\newcommand{\namedref}[2]{\hyperref[#2]{#1~\ref*{#2}}}

\newcommand{\WZ}{\text{WZ}}
\newcommand{\PS}{\text{PS}}
\newcommand{\AS}{\text{AS}}
\newcommand{\EQ}{\text{EQ}}
\newcommand{\GK}{\text{GK}}
\newcommand{\image}{\text{image}}

\newcommand{\Algorithmref}[1]{\namedref{Algorithm}{algo:#1}}
\newcommand{\Chapterref}[1]{\namedref{Chapter}{chap:#1}}
\newcommand{\Sectionref}[1]{\namedref{Section}{sec:#1}}
\newcommand{\Subsectionref}[1]{\namedref{Section}{subsec:#1}}
\newcommand{\Subsubsectionref}[1]{\namedref{Section}{subsubsec:#1}}
\newcommand{\Appendixref}[1]{\namedref{Appendix}{app:#1}}
\newcommand{\Theoremref}[1]{\namedref{Theorem}{thm:#1}}
\newcommand{\Corollaryref}[1]{\namedref{Corollary}{cor:#1}}
\newcommand{\Propositionref}[1]{\namedref{Proposition}{prop:#1}}
\newcommand{\Conjectureref}[1]{\namedref{Conjecture}{conj:#1}}
\newcommand{\Definitionref}[1]{\namedref{Definition}{defn:#1}}
\newcommand{\Lemmaref}[1]{\namedref{Lemma}{lem:#1}}
\newcommand{\Remarkref}[1]{\namedref{Remark}{remark:#1}}
\newcommand{\Claimref}[1]{\namedref{Claim}{claim:#1}}
\newcommand{\Factref}[1]{\namedref{Fact}{fact:#1}}
\newcommand{\Tableref}[1]{\namedref{Table}{tab:#1}}
\newcommand{\Figureref}[1]{\namedref{Figure}{fig:#1}}
\newcommand{\Equationref}[1]{\namedref{Equation}{eq:#1}}
\newcommand{\Footnoteref}[1]{\namedref{Footnote}{foot:#1}}
\newcommand{\Pageref}[1]{\hyperref[#1]{page~\pageref*{#1}}}



%%%%
\newcommand{\eps}{\ensuremath{\epsilon}\xspace}


\definecolor{darkred}{rgb}{0.5, 0, 0} 
\definecolor{darkblue}{rgb}{0,0,0.5} 

\hypersetup{
    colorlinks=true,
    linkcolor=darkred,
    citecolor=darkblue,
    urlcolor=darkblue   
}


\renewcommand{\ij}{\ensuremath{\vec{ij}}\xspace}
\newcommand{\ji}{\ensuremath{\vec{ji}}\xspace}
\newcommand{\Rplus}{\ensuremath{\mathbb{R}_+}\xspace}

\newcommand{\PinextA}{\ensuremath{\mathrm{next}^A_\Pi}\xspace}
\newcommand{\PinextB}{\ensuremath{\mathrm{next}^B_\Pi}\xspace}
\newcommand{\PioutA}{\ensuremath{\mathrm{out}^A_\Pi}\xspace}
\newcommand{\PioutB}{\ensuremath{\mathrm{out}^B_\Pi}\xspace}
\newcommand{\Piout}{\ensuremath{\mathrm{out}_\Pi}\xspace}
\newcommand{\Pipr}[1]{\ensuremath{\mathrm{Pr}_\Pi[#1]}\xspace}
\newcommand{\Pileft}{\ensuremath{\Pi^{(0)}}\xspace}
\newcommand{\Pileftpr}[1]{\ensuremath{\mathrm{Pr}_{\Pileft}[#1]}\xspace}
\newcommand{\fleft}{\ensuremath{f^{(0)}}\xspace}
\newcommand{\Xleft}{\ensuremath{\X^{(0)}}\xspace}
\newcommand{\rholeft}{\ensuremath{\rho^{(0)}}\xspace}
\newcommand{\sigmaleft}{\ensuremath{\sigma^{(0)}}\xspace}
\newcommand{\fright}{\ensuremath{f^{(1)}}\xspace}

\newcommand{\Pizeroout}{\ensuremath{\mathrm{out}_{\Pi_0}}\xspace}

\newcommand{\balpha}{\ensuremath{{\bf \alpha}}\xspace}
\newcommand{\bzero}{\ensuremath{{\bf 0}}\xspace}
\newcommand{\RI}{\ensuremath{RI}\xspace}
\newcommand{\supp}{\ensuremath{\textsf{supp}}\xspace}
\newcommand{\bb}{\ensuremath{{\bf b}}\xspace}
\newcommand{\doublebarbx}{\ensuremath{\bar{\bar{{\bf x}}}}\xspace}
\newcommand{\btb}{\ensuremath{\tilde{\bf b}}\xspace}
\newcommand{\bc}{\ensuremath{{\bf c}}\xspace}
\newcommand{\bd}{\ensuremath{{\bf d}}\xspace}
\newcommand{\be}{\ensuremath{{\bf e}}\xspace}
\newcommand{\bhe}{\ensuremath{\hat{\bf e}}\xspace}
\newcommand{\bte}{\ensuremath{\tilde{\bf e}}\xspace}
\newcommand{\bbf}{\ensuremath{{\bf f}}\xspace}
\newcommand{\btf}{\ensuremath{\tilde{\bf f}}\xspace}
\newcommand{\bg}{\ensuremath{{\bf g}}\xspace}
\newcommand{\br}{\ensuremath{{\bf r}}\xspace}
\newcommand{\btr}{\ensuremath{\tilde{\bf r}}\xspace}
\newcommand{\bx}{\ensuremath{{\bf x}}\xspace}
\newcommand{\bZ}{\ensuremath{{\bf Z}}\xspace}
\newcommand{\bp}{\ensuremath{{\bf p}}\xspace}
\newcommand{\barbp}{\ensuremath{\overline{\mathbf{p}}}\xspace}
\newcommand{\bwx}{\ensuremath{\widehat{\bf x}}\xspace}
\newcommand{\btx}{\ensuremath{\widetilde{\bf x}}\xspace}
\newcommand{\by}{\ensuremath{{\bf y}}\xspace}
\newcommand{\bty}{\ensuremath{\widetilde{\bf y}}\xspace}
\newcommand{\bz}{\ensuremath{{\bf z}}\xspace}
\newcommand{\bs}{\ensuremath{{\bf s}}\xspace}
\newcommand{\bts}{\ensuremath{\tilde{\bf s}}\xspace}
\newcommand{\bw}{\ensuremath{{\bf w}}\xspace}
\newcommand{\btw}{\ensuremath{\widetilde{\bf w}}\xspace}
\newcommand{\bu}{\ensuremath{{\bf u}}\xspace}
\newcommand{\bv}{\ensuremath{{\bf v}}\xspace}
\newcommand{\nr}{\ensuremath{{n_r}}\xspace}
\newcommand{\nc}{\ensuremath{{n_c}}\xspace}
\newcommand{\bA}{\ensuremath{{\bf A}}\xspace}
\newcommand{\bE}{\ensuremath{{\bf E}}\xspace}
\newcommand{\bF}{\ensuremath{{\bf F}}\xspace}
\newcommand{\bT}{\ensuremath{{\bf T}}\xspace}
\newcommand{\calS}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\bS}{\ensuremath{{\bf S}}\xspace}
\newcommand{\bV}{\ensuremath{{\bf V}}\xspace}
\newcommand{\btS}{\ensuremath{\tilde{\bf S}}\xspace}
\newcommand{\bX}{\ensuremath{{\bf X}}\xspace}
\newcommand{\bN}{\ensuremath{{\bf N}}\xspace}
\newcommand{\btX}{\ensuremath{\widetilde{\bf X}}\xspace}
\newcommand{\out}[1]{\ensuremath{\Pi^{\text{out}}_{#1}}\xspace}
\newcommand{\A}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\B}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\C}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\bbE}{\ensuremath{\mathbb{E}}\xspace}
\newcommand{\calO}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\I}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\calP}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\Y}{\ensuremath{\mathcal{Y}}\xspace}
\newcommand{\Z}{\ensuremath{\mathcal{Z}}\xspace}
\newcommand{\U}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\V}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\W}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\M}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\N}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\setS}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\E}{\ensuremath{\mathcal{E}}\xspace}
\newcommand{\G}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\R}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\T}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\bbZ}{\ensuremath{\mathbb{Z}}\xspace}
\newcommand{\equi}{\ensuremath{\triangleleft}\xspace}
\newcommand{\mx}{\ensuremath{\mathsf{Max}}\xspace}
\newcommand{\MaxTerm}{\ensuremath{\mathrm{MaxTerm}}\xspace}
\newcommand{\tmx}{\ensuremath{\mathsf{\widetilde{Max}}}\xspace}

\newcommand{\jbar}{\ensuremath{{\bar{\jmath}}}\xspace}
\newcommand{\zz}[1]{{\color{gray}\ensuremath{z_{#1}}}\xspace}



\newcommand{\twobythreetable}[8]{%
\protect{\begin{tabular}{|c|ccc|}\hline & $#1_1$ & $#1_2$ & $#1_3$  \\\hline $#2_1$ & #3 & #4 & #5 \\ $#2_2$ & #6 & #7 & #8\\\hline\end{tabular}}}


\renewcommand{\paragraph}[1]{\smallskip\noindent{\bf #1}~}

\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}


==> organization.tex <==
In \Sectionref{shapley} we provide a brief understanding of Shapley values and the form in which they are useful as interpretations for a predictive model. \Sectionref{noi} emphasizes on clearly defining our expectations before we use a method for generating interpretations. We discuss three different natures of interpretation and the formal analysis accompanying each one of them. In \Sectionref{moi}, we study different useful measures of interpretation which when used in conjunction with the different natures of interpretation from \Sectionref{noi} demystifies the implications of what these interpretations actually signify. The usefulness of this framework of interpretability is seen in two use cases, (i) deriving insights for the model output, (ii) deriving insights for the predictive performance of a model. We present numerical results in \Sectionref{results} which demonstrate the usefulness of different interpretability measures and a concluding note in \Sectionref{conclusion}. 
